Neural Subnetwork Ensembles

Neural network ensembles have been effectively used to improve generalization by combining the predictions of multiple independently trained models. However, the growing scale and complexity of deep neural networks have led to these methods becoming prohibitively expensive and time consuming to implement. Low-cost ensemble methods have become increasingly important as they can alleviate the need to train multiple models from scratch while retaining the generalization benefits that traditional ensemble learning methods afford. This dissertation introduces and formalizes a low-cost framework for constructing Subnetwork Ensembles, where a collection of child networks are formed by sampling, perturbing, and optimizing subnetworks from a trained parent model. We explore several distinct methodologies for generating child networks and we evaluate their efficacy through a variety of ablation studies and established benchmarks. Our findings reveal that this approach can greatly improve training efficiency, parametric utilization, and generalization performance while minimizing computational cost. Subnetwork Ensembles offer a compelling framework for exploring how we can build better systems by leveraging the unrealized potential of deep neural networks.

==> chapters/experiments.tex <==
\section{Noisy Subnetwork Ensembles}
\subsection{Ablations}
\subsubsection{Decision Boundaries}

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/noisy/decision-boundaries.pdf}
    \caption{The images above detail decision boundaries for a trained three layer multilayer perceptron after being perturbed with various mutations. With dense perturbations, there is a comparatively small window between a functional decision boundary and complete performance collapse. As mutations become more sparse, the model is better able to retain its behavior while the strength of parameter mutation increases.}
\end{figure}

We begin by exploring the interplay between mutation sparsity and mutation strength by visualizing how changing these values affects network predictions.
We use a simple three layer fully connected multilayer perceptron that contains 64 neurons in each layer.
We train this model on a binary interleaved spiral dataset that contains 2500 sample (x, y) points. 
We train for 10 epochs using the Adam optimizer \cite{kingma2017adam} with a learning rate $0.001$ and use this trained model as the starting point for all mutations.

We then perturb the model with mutations sampled from a Gaussian Distribution $N \sim \mathcal{N}(0, \sigma^2)$ where $\sigma$ corresponds to the mutation strength and with a mask sampled from a Bernoulli distribution $M \sim \text{Bernoulli}(\rho)$ where $\rho$ governs the probability of mutation sparsity. We ablate these hyperparameters from mutation strengths of $\sigma \in [0.05, 0.25]$ and mutation sparsities of $\rho \in [0.0, 0.9]$.

Using the perturbed models, we make predictions on a holdout test set containing 250 samples. In figure 4.2, we display a grid of the decision boundaries of these perturbed models on the test set as we ablate between mutation strength and sparsity.
When mutations are dense, we see a very quick collapse of performance for small perturbations. The window for optimal dense mutation is quite small even for this toy network and simple dataset. When mutations become more sparse, the model is able to maintain a good classification boundaries while displaying small variations of prediction diversity. This kind of behavior is desirable for neuroevolutionary populations as ensemble learning research has shown that populations perform better with large numbers of both accurate and diverse members \cite{bonab2016theoretical}.



\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/noisy/c10-ablations.pdf}
    \includegraphics[width=\textwidth]{figures/noisy/c100-ablations.pdf}
    \caption{Results of mutation ablations on a trained WideResNet-28x10 model on CIFAR-10 and CIFAR-100. Lines of different colors correspond to the percentage of sparsity for the mutations. Dashed lines correspond to static subspace evolution while solid lines correspond to dynamic subspace evolution. The left most graph reports the average KL divergence. The middle graph reports the accuracy of an averaged model of the four top candidates after one generation of evolution. The rightmost graph reports accuracy if you treat those four models as an ensemble.}
\vspace{0.1in}
\end{figure}

\subsubsection{Wide Resnets}

Next, we aim to explore whether the intuitions about how mutations affect predictions translate to a much larger convolutional network on benchmark computer vision datasets.
For this experiment, we conduct ablations on the CIFAR-10 and CIFAR-100 datasets \cite{Krizhevsky09learningmultiple}. These are popular benchmark datasets and their use is widespread in computer vision research. They each contain 50,000 training and 10,000 test samples of colored 32x32 pixel images. CIFAR-10 contains samples belonging to one of 10 classes while CIFAR-100 contains samples belonging to one of 100 classes.
We use a WideResNet-28x10 model for our parent network, which is a highly accurate network architecture that contains $\sim 36M$ parameters. This network is a variant on the popular ResNet that decreases the depth and increases the width of each convolutional layer \cite{https://doi.org/10.48550/arxiv.1605.07146}.

We implement a standard training algorithm for this type of model where we train for 100 epochs using Stochastic Gradient Descent with Nestorov momentum \cite{sutskever13nesterov}.
A stepwise learning rate decay is used where an inital value of 0.1 decays to 0.01 after 50\% of training and decays again to 0.001 for the final 10\% of training.
We use standard data augmentation schemes for CIFAR that includes a random crop and random horizontal flip along with mean standard normalization.
We split the test set in half in order to conduct a validation set used for model selection.

The parent networks achieve an accuracy of approximately 96\% on CIFAR-10 and approximately 80\% on CIFAR-100.
Using these saved models as parent networks, we then perturb the models with varying amounts of mutation strengths, $\sigma \in (0.0, 0.05]$, and sparsities, $\rho \in [0.01, 0.99]$, and we evaluate their performance on the test sets.

Figure 3 displays the results of these experiments on CIFAR-10 where we start by measuring the effect that mutations have on KL Divergence.
Predictably, we see that KL divergence quickly increases as the density and strength of mutations increase.
The rapid increase in KL divergence for dense perturbations illustrates how quickly performance collapses between very small changes in mutation strength.

We then implement a single evolutionary generation where a population of 16 models are created by perturbing the parent model according to a given mutation strength and sparsity.
The top 4 models with the best accuracy on the validation set are then selected and evaluated.
We then report accuracy on the test set where the weights of the top 4 models are averaged together.
We also evaluate these four models as if they were part of an ensemble, where each model is evaluated independently and their predictions are combined.
The averaged weights model is much more consistent compared to the ensemble which displays large amounts of variance for strong mutations.
While the differences are small in this case, ensembles tend to slightly outperform averaged weight models for lower levels of mutation strengths (where individual model accuracy is higher) while averaged models outperform ensembles for higher levels of mutation (where individual model performance is worse).

We repeat the above experiments with both static and dynamic subspace evolution.
For static subspace evolution, we mutate the same subnetwork for each generated member in the population. For dynamic subspace evolution, each child is mutated with a random subnetwork mask. On this task, we see little difference between static and dynamic subspaces, suggesting that the specific subnetwork that we mutate does not matter in the context of both averaged and ensemble evaluations.

\subsection{Benchmarks}

\begin{table}
\scriptsize
\begin{tabularx}{\textwidth}{X l l l l l l c c c c c}
\toprule
Model & Acc $\uparrow$ & NLL $\downarrow$ & ECE $\downarrow$ & eAcc $\uparrow$ & eNLL $\downarrow$ & eECE $\downarrow$ & $\Delta$Acc $\uparrow$ & Parameters & \multicolumn{1}{c}{$\sigma$} & \multicolumn{1}{c}{$\rho$} & $\overline{KL}$  \\
\midrule
AlexNet & 56.46 & 1.904 & 0.021 & 56.52 & 1.903 & 0.019 & 0.06 & 61.1M & 0.006 & 0.80 & 0.038 \\
\text{DenseNet-121} & 74.43 & 1.014 & 0.024 & 74.68 & 1.004 & 0.021 & 0.25 & 8.0M & 0.007 & 0.85 & 0.077 \\
\text{Inception-V3} & 69.57 & 1.819 & 0.184 & 69.98 & 1.681 & 0.169 & 0.41 & 27.2M & 0.008 & 0.90 & 0.037 \\
\text{MobileNet-V2} & 72.12 & 1.136 & 0.072 & 72.14 & 1.132 & 0.024 & 0.02 & 3.5M & 0.007 & 0.90 & 0.085 \\
\text{ResNet-18}  & 69.76 & 1.247 & 0.026 & 69.93 & 1.238 & 0.022 & 0.17 & 11.7M & 0.010 & 0.90 & 0.060 \\
\text{ResNext-50} & 77.64 & 0.945 & 0.065 & 77.72 & 0.929 & 0.059 & 0.08 & 25.0M & 0.005 & 0.80 & 0.051 \\
\text{ShuffleNet-V2} & 69.51 & 1.354 & 0.072 & 69.57 & 1.351 & 0.071 & 0.06 & 2.3M & 0.012 & 0.95 & 0.052 \\
SqueezeNet & 58.10 & 1.852 & 0.017 & 58.14 & 1.852 & 0.017 & 0.04 & 1.2M & 0.007 & 0.75 & 0.072 \\
\text{VGG-16} & 71.62 & 1.140 & 0.027 & 71.64 & 1.138 & 0.028 & 0.02 & 138.4M & 0.010 & 0.95 & 0.019\\
\text{WideResNet-50} & 78.47 & 0.879 & 0.054 & 78.60 & 0.852 & 0.038 & 0.13 & 68.9M & 0.011 & 0.90 & 0.178 \\
\bottomrule
\end{tabularx}
\caption{Results for sparse mutation ensembles on ImageNet with a wide variety of models. Mutation sparsity and strength are determined from a small hyperparameter grid search. Accuracy (Acc), Negative Log Likelihood (NLL), and expected calibration error (ECE) are reported for the parent and the ensemble. Metrics prepended with $e$ refer to the ensemble results. $\Delta$Acc is the change in accuracy between the parent and the ensemble, $\sigma$ is the mutation strength, $\rho$ is the mutation sparsity, and $\overline{KL}$ is the average output divergence between the mutated models and the parent models. 16 models are generated and the 8 most accurate candidates on a validation set are used together as an ensemble.}
\end{table}

We then explore our approach on the difficult benchmark computer vision dataset, ImageNet \cite{NIPS2012_c399862d}. ImageNet is a large scale collection of images that have been hand labelled for use in machine learning tasks and is organized according to the wordnet dataset hierarchy. Over 14 million images and 20,000 labels have been collected in total. We use the 2012 ImageNet collection which consists of a training set of 1.2 million images and a validation set of 50,000 images, each belonging to one of 1000 categories. Images have varying sizes and aspect ratios and consist of both colored and grayscale photos. We normalize all images are normalized with mean and standard deviation scaling and we implement standard data augmentation which consists of resizing to 256x256 pixels and center cropping to 224x224 pixels.

We evaluate our approach with ten popular deep neural network architectures of varying sizes and generalization capacities in order to demonstrate the generality and power of our approach in many different contexts. All networks are pretrained and available from the torchvision repository \cite{torchvision}. 

We break the ILSVRC 2012 set of 50,000 images into a 50/50 split between validation and test sets that each contain 25,000 samples.
All fitness evaluations and model selections use the validation set and all reported results are evaluated on the holdout test set.

We report accuracy, negative log likelihood, and estimated calibration error for the parent network and our evolutionary ensemble. We run each model twice and report the best results.

We conduct a hyperparameter grid search in order to find appropriate hyperparameter values for mutation strength and sparsity for each model.
Using a separate holdout dataset of 1000 samples we measure the average KL Divergence and accuracy while we ablate sparsity $\rho \in [0.5, 0.99]$ and mutation strength $\sigma \in [0.001, 0.015]$. We then choose both a mutation strength and sparsity value that maximizes accuracy while targeting a KL Divergence of $\sim 0.05$. This value was found to be an empirically safe option for most models, balancing the accuracy of candidate models with exploration to reliably improve generalization performance when candidates are combined.

Using the sparse mutation hyperparameters found from the short grid search, a population of 16 models are created with mirrored sampling.
Each is evaluated on a validation set and the top 8 candidates with the best accuracy are selected.
We then evaluate the top 8 candidates independently and combine their predicted probabilities as if they were part of an ensemble and report the accuracy, negative log likelihood and expected calibration error.

Table I contains both the parent results and the ensemble results. From only one generation of evolutionary tuning, we see consistent improvement in all metrics for each model. While the difference between generalization performance is very small in many cases, it is notable that convergence is extremely stable and appears to be monotonic with optimal mutation hyperparameters. We don't observe the noisy oscillations you'd commonly see with fine tuning using stochastic gradient descent.
There's also a question of how much potential is able to be squeezed out of the fully trained networks. There is no accepted method for determining the theoretical ceiling of generalization capacity for complex network architectures.
It is possible that these small improvements are significant in the grand scheme of things where an improvement of 0.5\% accuracy on a dataset of 50,000 images corresponds to 250 more correct predictions, which can be significant in some contexts.
It is notable that our results only incorporate a single generation of evolutionary fine tuning and future research with more iterations and more thorough hyperparameter searches will likely improve performance further.

\subsubsection{Procgen}

% Run stuff here!! train_procgen repo***

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/noisy/procgen-screenshot.png}
    \caption{Placelholder image for procgen results.}
\end{figure}


\subsection{Discussion}

We introduce noisy subnetwork ensembles as an approach to alleviating the challenges of mutating deep neural networks by breaking up dense mutations into low-dimensional subspaces. This widens the critical mutation window, which can significantly reduce the variance as children in evolutionary populations can handle stronger perturbations before performance collapse. We explore how these sparse mutations can be implemented with a standard neuroevolutionary method in order to fine-tune and further optimize pre-trained networks and we show how ensembles of the top candidates in a population can aid in generalization.

We conduct several ablation studies in order to explore the interplay between sparsity and mutation strength on network behavior. We conduct a decision boundary experiment where visualizations are created that show the predictions of a model on a binary classification dataset. After being perturbed with dense mutations, the model sees a rapid decline in performance while sparsity significantly helps in maintaining accurate predictions while encouraging diverse representation. We then explore how these insights translate to a wide residual network on CIFAR where we explore parameter sensitivity, static/dynamic subspace evolution, and the differences between averaged model performance and population ensemble performance as result of different levels of mutation strength and sparsity. Our findings reaffirm the idea that sparse mutations produce more accurate models more reliably than dense mutations.

We then introduce the first large scale exploration of evolutionary fine tuning with sparse mutations on ImageNet with a wide variety of deep neural network architectures.
We use a relatively small population of 16 models in which the top 8 most accurate on a validation set are selected and evaluated together as an ensemble.
Our approach reliably and consistently improves performance on every model with only a single evolutionary generation.

\section{Sparse Subnetwork Ensembles}
\subsection{Ablations}

\begin{figure}
    \centering
    \includegraphics[width=.45\textwidth]{figures/sparse/sparsity-new.pdf}
    \includegraphics[width=.45\textwidth]{figures/sparse/neuron-elimination-new.pdf}
    \includegraphics[width=.45\textwidth]{figures/sparse/tuning-new.pdf}
    \includegraphics[width=.45\textwidth]{figures/sparse/population-new.pdf}

\caption{Hyperparameter ablations on CIFAR-10/CIFAR-100 with various LeNet configurations. The first figure reports the effect of sparsity on ensemble performance for models of different size. The second compares neuron and connection elimination for the large model. The third figure explores both random/anti-random pruning and constant/cyclic tuning schedules over 10 runs. The final figure evaluates the effect of ensemble size up to $M=128$.}
\end{figure}


We explore the impact of several hyperaparameters on our ensembles, including: amount of sparsity, random/anti-random pruning, connection/neuron elimination, constant/cyclic tuning schedule and ensemble size. We use variations of the LeNet-5 model architecture where we vary the number of neurons in each hidden layer. We call these small, medium and large models the {\it LeNet-S} (253,290 parameters), {\it LeNet-M} (1,007,306 parameters), and {\it LeNet-L} versions (4,017,546 parameters). See appendix for additional details on the layer configurations.

We conduct our experiments on CIFAR-10 and CIFAR-100. We use Stochastic Gradient Descent (SGD) with Nesterov momentum for our evaluation of random/anti-random pruning and constant/cyclic tuning schedule. We use an initial learning rate of $\eta_1 = 0.1$ for 50\% of the training budget which decays linearly to $\eta_2 = 0.001$ at 90\% of the training budget. The learning rate is kept constant at $\eta_2 = 0.001$ for the final 10\% of training. Children are tuned with either a constant learning rate of $\eta=0.01$ for 5 epochs or with a one-cycle schedule that ramps up from $\eta_1=0.001$ to $\eta_2=0.1$ at 10\% of tuning, then decaying to $\eta_3=1e-7$ at the end of 5 epochs. For all other experiments, we use ADAM with a learning rate of $\eta = 0.001$.

To evaluate sparsity, we take each model variation ({\it LeNet-S}, {\it LeNet-M}, and {\it LeNet-L}) and train the parent network for 8 epochs. An ensemble of 8 children are created that are each tuned for 3 epochs. We report the ensemble accuracy at both 1 and 3 epochs of tuning for child sparsity ranging from 10\% to 90\%. 
All models are pruned using global connection elimination. 

To evaluate neuron and connection elimination, we train the {\it LeNet-L} parent network for 8 epochs. An ensemble of 8 children is created, where each is pruned using either connection or neuron elimination. Each child is tuned for 3 epochs. We report ensemble accuracy for both neuron and connection elimination at various levels of sparsity between 10\% and 90\%.

To evaluate ensemble size, we take the {\it LeNet-M} network and produce up to 128 candidate member networks using 50\% sparsity connection pruning and 1 epoch of constant rate tuning ($\eta=0.001$). We evaluate ensemble performance over 10 runs as we increase the size of the ensemble from 4 to 128.

We finally evaluate random/anti-random pruning and constant/cyclic tuning. We use the {\it LeNet-L} network and create an ensemble of two models using each combination of random (R) or anti-random (AR) pruning and constant fine-tuning (FT) or one-cycle tuning (1C). We record results for 10 sample runs of each configuration.

Figure 3 shows the results of all ablation experiments. The leftmost figure illustrates the capacity that larger models have for learning more efficiently. Ensemble accuracy improves up to a critical region as child networks become more sparse, {\em without any additional epochs of training}. This indicates that more sparsity can yield greater diversity in the ensemble. 

The second figure shows that connection pruning allows for more sparsity when compared to neuron pruning. We see no difference in performance for sparsity values up to 50\%, but we note that the performance collapses for neuron pruning much sooner than for connection pruning.

The third figure shows that the combination of anti-random pruning and one-cycle tuning outperforms other configurations. We see significant evidence of enhanced diversity between two models with the addition of these two techniques on both CIFAR-10 and CIFAR-100.

The rightmost figure shows that ensembles consistently perform better as we increase the number of ensemble members. These results suggest significant advantages in using methods that can dynamically generate ensemble members, as performance monotonically increases with size.


\subsection{Benchmarks}

Ensemble learning literature has not focused on evaluating approaches for very small training budgets, but we believe there is significant value in doing so. We take inspiration from Stanford's DAWNBench experiment, the goal of which is to train a single model to a target accuracy in as little time as possible \cite{coleman2017DAWNBench}. Thus, we conduct a comparison among methods that limits the total training budget to only 16 epochs.
Each method is ran with a sample size of 10 runs, except for both versions of Prune and Tune, which are ran 30 times each.

The {\bf Independent Model} is a standard neural network model trained for all 16 epochs.
The {\bf Bagged Ensemble} contains 8 full size models, each trained for two epochs. Each member is trained on a 90\% sample of the full training set.
The {\bf Dropout Model} is identical to the Independent Model except dropout layers are inserted after every convolutional and linear layer.
These dropout layers use the same 50\% sparsity value that we use for Prune and Tune, to keep the number of parameters consistent. For {\bf Prune and Tune}, we train a single parent network for 8 epochs, we then create 8 children using random connection pruning with a 50\% sparsity target. For {\bf Prune and Tune (AR)} we create 8 children using anti-random (AR) pruning: we create 4 pairs of network/anti-networks each with 50\% sparsity.  We fine tune each child for only 1 epoch. Each approach uses the ADAM optimizer with a fixed learning rate of $\eta=0.001$.

We report the mean accuracy and standard error achieved for each method in Table 1. One may be surprised by the poor performance of Dropout. A 50\% dropout rate is larger than typical configurations, but we chose to do this to closely match the configuration of Prune and Tune Ensemble children. This combined with the small budget leads to a much slower convergence for these models. This experiment is designed to create an initial baseline for small training budgets that can be further explored in future work.

In these small fixed training budget experiments, comparisons using a simple t-test shows that the Prune and Tune ensemble methods are significantly better than all other methods (at p=0.0001) over 30 runs.

\begin{table}
\small

\begin{tabularx}{\columnwidth}{l X c c}
\toprule
Model & Method & CIFAR-10 & CIFAR-100 \\
\midrule
LeNet-L  & Independent & 70.29 $\pm$ 0.21 & 34.39 $\pm$ 0.18 \\
        & Dropout & 70.06 $\pm$ 0.32  & 28.98 $\pm$ 0.33 \\
        & Bagged & 70.97 $\pm$ 0.13  & 32.40 $\pm$ 0.11 \\
        & PAT (R) & 75.51 $\pm$ 0.06  & 41.68 $\pm$ 0.14 \\
        & PAT (AR) & \textbf{75.75} $\pm$ \textbf{0.06} & \textbf{41.85} $\pm$ \textbf{0.13} \\
\midrule
ResNet-18 & Independent & 80.99 $\pm$ 0.11 & 49.26 $\pm$ 0.09 \\
        & Dropout & 72.97 $\pm$ 0.41 & 37.69 $\pm$ 0.28 \\
        & Bagged & 79.88 $\pm$ 0.05 & 46.18 $\pm$ 0.06 \\
        & PAT (R) & 84.61 $\pm$ 0.07  & 57.08 $\pm$ 0.07 \\
        & PAT (AR) & \textbf{84.68} $\pm$ \textbf{0.04} & \textbf{57.26} $\pm$ \textbf{0.06} \\
\midrule
DenseNet-121 & Independent & 84.14 $\pm$ 0.09 & 56.62 $\pm$ 0.09 \\
          & Dropout & 79.59 $\pm$ 0.36 & 44.02 $\pm$ 0.58 \\
          & Bagged & 81.16 $\pm$ 0.04 & 48.48 $\pm$ 0.06 \\
          & PAT (R) & 86.26 $\pm$ 0.07  & 62.02 $\pm$ 0.07 \\
            & PAT (AR) & \textbf{86.35} $\pm$ \textbf{0.04} & \textbf{62.09} $\pm$ \textbf{0.06} \\
\bottomrule
\end{tabularx}

\caption{Accuracy of various methods for 16 epochs of training. Ensembles contain eight models.}\label{tab:low-budget-table}
\end{table}

\subsubsection{Decompositional Efficiency}

% Compare to mothernets. It's more efficient to train big and then prune as opposed to mothernets which train small and then grow.

We compare our method to the current state-of-the-art rapid ensembling algorithm, MotherNets. Conceptually, our methods are quite similar. MotherNets start with a small shared structure and tunes an ensemble of larger children. Prune and Tune starts with a large parent and tunes an ensemble of smaller children. Ultimately, we want to explore which approach is more efficient.

We use fully connected networks and the Net2Net \cite{chen2016net2net} algorithm to hatch the mothernet children, which is suggested in the original paper \cite{wasay2020mothernets}.

We conduct a simplified experiment on the small benchmark dataset MNIST, which is a collection of small handwritten black and white digits \cite{lecun1998mnist}. 

We start with a MotherNet with one hidden layer of 16 neurons. We hatch a child that grows its hidden layer to 32 neurons. We compare this with a Prune and Tune Parent that contains a single hidden layer of 64 neurons. We then create a child by pruning its hidden layer to 32 neurons. We train both parents and the resulting children for ten epochs each and we conduct this experiment with two different optimizers. One with the Adam optimizer \cite{kingma2017adam} and one with Stochastic Gradient Descent with Momentum \cite{rumelhart1986learning}. Both resulting children are the same size and both approaches use the same number of training epochs.

\begin{figure}
\includegraphics[width=\columnwidth]{figures/sparse/mothernets.png}
\caption{Early training efficiency of mothernets vs prune and tune with both SGD and Adam.}
\end{figure}

Prune and Tune Ensembles reach higher accuracies than MotherNets in fewer epochs. We see a smooth and consistent training curve with the hatched children of MotherNets, while Prune and Tune children undergo a large drop in accuracy before quickly recovering and exceeding the performance of the MotherNet children.

One benefit to MotherNets, is the ability to dynamically add more parameters if needed. The size of Prune and Tune Ensemble children are inherently constrained by the size of the parent network. Assuming we start off with a large enough parent network, we see improved training efficiency with Prune and Tune Ensembles when compared to MotherNets. This suggests the possibility of establishing a new Pareto frontier for the training-time/accuracy trade-off.


\begin{table}
\scriptsize

\begin{tabularx}{\textwidth}{X l l l l l l c c}
\toprule
Methods (CIFAR-10/WRN-28-10) & Acc $\uparrow$ & NLL $\downarrow$ & ECE $\downarrow$ & cAcc $\uparrow$ & cNLL $\downarrow$ & cECE $\downarrow$ & FLOPs $\downarrow$ & Epochs $\downarrow$ \\
\midrule
Independent Model$^*$ & 96.0 & 0.159 & 0.023 & 76.1 & 1.050 & 0.153 & 3.6e17 & 200 \\
Monte Carlo Dropout$^*$ & 95.9 & 0.160 & 0.024 & 68.8 & 1.270 & 0.166 & 1.00x & 200 \\
TreeNet (M=3)$^*$ & 95.9 & 0.258 & 0.018 & 75.5 & {\bf 0.969} & 0.137 & 1.52x & 250 \\
SSE (M=5) & 96.3 & 0.131 & 0.015 & 76.0 & 1.060 & 0.121 & 1.00x & 200 \\
FGE (M=12) & 96.3 & 0.126 & 0.015 & 75.4 & 1.157 & 0.122 & 1.00x & 200 \\
PAT (M=6) (AR + 1C) & {\bf 96.48} & {\bf 0.113} & {\bf 0.005} & {\bf 76.23} & 0.972 & {\bf 0.081} & {\bf 0.85x} & {\bf 200} \\
\midrule
BatchEnsemble (M=4)$^*$ & 96.2 & 0.143 & 0.021 & 77.5 & 1.020 & 0.129 & 4.40x & 250 \\
MIMO (M=3)$^*$ & 96.4 & 0.123 & 0.010 & 76.6 & 0.927 & 0.112 & 4.00x & 250 \\
EDST (M=7)$^*$ & 96.4 & 0.127 & 0.012 & 76.7 & 0.880 & 0.100 & 0.57x & 850 \\
DST (M=3)$^*$ & 96.4 & 0.124 & 0.011 & 77.6 & 0.840 & 0.090 & 1.01x & 750 \\
Dense Ensemble (M=4)$^*$ & 96.6 & 0.114 & 0.010 & 77.9 & 0.810 & 0.087 & 1.00x & 800 \\
\bottomrule
\end{tabularx}

\vspace{0.2in}


\begin{tabularx}{\textwidth}{X l l l l l l c c }
\toprule
Methods (CIFAR-100/WRN-28-10) & Acc $\uparrow$ & NLL $\downarrow$ & ECE $\downarrow$ & cAcc $\uparrow$ & cNLL $\downarrow$ & cECE $\downarrow$ & FLOPs $\downarrow$ & Epochs $\downarrow$ \\
\midrule
Independent Model$^*$ & 79.8 & 0.875 & 0.086 & 51.4 & 2.700 & 0.239 & 3.6e17 & 200 \\
Monte Carlo Dropout$^*$ & 79.6 & 0.830 & 0.050 & 42.6 & 2.900 & 0.202 & 1.00x & 200 \\
TreeNet (M=3)$^*$ & 80.8 & 0.777 & 0.047 & {\bf 53.5} & {\bf 2.295} & 0.176 & 1.52x & 250 \\
SSE (M=5) & 82.1 & 0.661 & 0.040 & 52.2 & 2.595 & 0.145 & 1.00x & 200 \\
FGE (M=12) & 82.3 & 0.653 & 0.038 & 51.7 & 2.638 & 0.137 & 1.00x & 200 \\
PAT (M=6) (AR + 1C) & {\bf 82.67} & {\bf 0.634} & {\bf 0.013} & 52.70 & 2.487 & {\bf 0.131} & {\bf 0.85x} & {\bf 200} \\
\midrule
BatchEnsemble (M=4)$^*$ & 81.5 & 0.740 & 0.056 & 54.1 & 2.490 & 0.191 & 4.40x & 250 \\
MIMO (M=3)$^*$ & 82.0 & 0.690 & 0.022 & 53.7 & 2.284 & 0.129 & 4.00x & 250 \\
EDST (M=7)$^*$ & 82.6 & 0.653 & 0.036 & 52.7 & 2.410 & 0.170 & 0.57x & 850 \\
DST (M=3)$^*$ & 82.8 & 0.633 & 0.026 & 54.3 & 2.280 & 0.140 & 1.01x & 750 \\
Dense Ensemble (M=4)$^*$ & 82.7 & 0.666 & 0.021 & 54.1 & 2.270 & 0.138 & 1.00x & 800 \\
\bottomrule
\end{tabularx}

\caption{Results for ensembles of WideResNet-28-10 models on both CIFAR-10 and CIFAR-100. Methods with $^*$ denote results obtained from \cite{havasi2021training, liu2021freetickets}. Best low-cost ensemble results are {\bf bold}. cAcc, cNLL, and cECE correspond to corrupted test sets. We report the mean values over 10 runs for PAT.}
\end{table}

We next evaluate Prune and Tune Ensembles with a larger training budget of 200 epochs with WideResNet-28-10. We take the training configuration, ensemble size and parameter setting directly from studies of three state-of-the-art low-cost ensemble methods: MotherNets \cite{wasay2020mothernets}, Snapshot Ensembles \cite{huang2017snapshot}, and Fast Geometric Ensembles \cite{garipov2018loss}. We also compare our results with published results of several recent low-cost ensemble methods including: TreeNets \cite{lee2015m}, BatchEnsemble \cite{wen2020batchensemble}, FreeTickets \cite{liu2021freetickets}, and MIMO \cite{havasi2021training}.

All methods compared use WideResNet-28-10 and Stochastic Gradient Descent with Nesterov momentum $\mu=0.9$ and weight decay $\gamma=0.0005$ \cite{sutskever13nesterov}. The Prune and Tune ensemble size and training schedule is as used in previous comparisons \cite{wasay2020mothernets, garipov2018loss}.  We use a batch size of 128 for training and use random crop, random horizontal flip, and mean standard scaling data augmentations for all approaches \cite{garipov2018loss, havasi2021training, liu2021freetickets, huang2017snapshot}. The parent learning rate uses a step-wise decay schedule. An initial learning rate of $\eta_1=0.1$ is used for 50\% of the training budget which decays linearly to $\eta_2=0.001$ at 90\% of the training budget. The learning rate is kept constant at $\eta_2=0.001$ for the final 10\% of training. 

The {\bf Independent Model} is a single WideResNet-28-10 model trained for 200 Epochs. The {\bf Dropout Model} includes dropout layers between convolutional layers in the residual blocks at a rate of 30\% \cite{zagoruyko2017wide}. {\bf Snapshot Ensembles} (SSE) use a cosine annealing learning rate with an initial learning rate $\eta = 0.1$ for a cycle length of 40 epochs \cite{huang2017snapshot}. {\bf Fast Geometric Ensembles} (FGE) use a pre-training routine for 156 epochs. A curve finding algorithm then runs for 22 epochs with a cycle length of 4, each starting from checkpoints at epoch 120 and 156. {\bf TreeNets}, \cite{lee2015m}, {\bf BatchEnsemble} \cite{wen2020batchensemble} and {\bf MIMO} \cite{havasi2021training} are all trained for 250 epochs. {\bf FreeTickets} introduces several configurations for building ensembles. We include their two best configurations for Dynamic Sparse Training (DST, M=3, S=0.8) and Efficient Dynamic Sparse Training (EDST, M=7, S=0.9).

{\bf Prune and Tune Ensembles} (PAT) train a single parent network for 140 epochs. Six children are created with anti-random pruning (50\% sparsity) and tuned with a one-cycle learning rate for 10 epochs. The tuning schedule starts at $\eta_1=0.001$, increases to $\eta_2=0.1$ at 1 epoch and then decays to $\eta_3=1e-7$ using cosine annealing for the final 9 epochs.

There is the potential to further improve performance by exploring larger ensemble sizes and different ratios of parent to child training time.

We report the mean accuracy (Acc), negative log likelihood (NLL), and expected calibration error (ECE) over 10 runs on both CIFAR-10 and CIFAR-100 along with their corrupted variants \cite{nado2021uncertainty, hendrycks2019robustness}. We also report the total number of floating point operations (FLOPs) and epochs used for training each method. We organize our tables into two groups based on training cost. The first group consists of low-cost training methods that take approximately as long as a single network would take to train. The second group of methods use either significantly more epochs or compute per epoch to achieve comparable performance. MIMO and BatchEnsemble both make use of batch repetition to train on more data while keeping the number of epochs low. FreeTickets (DST and EDST) use very sparse networks to keep FLOP counts low while using many more training epochs.

Prune and Tune Ensembles (using anti-random pruning and one-cycle tuning) outperform all low-cost ensemble methods and are competitive with methods that train for significantly longer. Our approach produces well calibrated, robust and diverse ensembles with excellent performance on out of distribution corrupted datasets.


\subsection{Discussion}

The Prune and Tune Ensemble algorithm is flexible and enables the creation of diverse and accurate ensembles at a significantly reduced computational cost. We do this by 1) training a single large parent network, 2) creating child networks by copying the parent and significantly pruning them using random or anti-random sampling strategies, and 3) fine tuning each of the child networks for a small number of training epochs.

With the experiments introduced here, Prune and Tune Ensembles outperform low-cost ensembling approaches on benchmark image classification datasets with a variety of popular deep neural network architectures. Our approach achieves comparable accuracy to ensembles that are trained on 4-5x more data. Prune and Tune Ensembles not only improve upon the training-time/accuracy trade-off, but also reduce memory and computational cost thanks to the use of sparse child networks.

Prune and Tune Ensembles can offer a new lens through which we can analyze generalization and diversity among subcomponents of deep neural networks. We hope to further explore larger scale benchmarks, anti-random pruning methodologies and applications to new problem domains in future work.


==> chapters/temp-stochastic-subnetwork-ensembles.tex <==
\section{Introduction}

...

\section{Implementation}

Our evaluations of subnetwork ensembles focus on static subnetworks with binary bit masks. We additionally propose a novel technique for representing neural subnetworks with probabilistic masks, where each parameter is assigned a score that determines how likely it is that a subnetwork parameter is retained on every forward pass. This introduces stochasticity into the subnetwork sampling process, which can act as a form of implicit regularization analagous to dropout. In some sense, this technique allows each child network to explore a larger space of subnetworks, preventing it from becoming overly reliant on a single fixed subnetwork configuration.

Consider a weight matrix $W \in \mathbb{R}^{m \times n}$ representing the weights of a particular layer in a neural network. We then introduce a probability matrix $P \in \mathbb{R}^{m \times n}$ containing scores that represent the probability that a parameter $W_{ij}$ will be will be masked on any given forward pass. The subnetwork mask $M \in \{0,1\}^{m \times n}$ is determined with a Bernoulli realization of the probability matrix $P$. 

The probability matrix can be generated in arbitrary ways. For example, a uniform distribution $P \sim U([0,1])^{m \times n}$ can be used to create subnetworks with a lot of variability. The ideas of neural partitioning naturally extend to anti-probability matrices $P' = 1 - P$ for creating opposed sets of probabilistic subnetworks.
%
\[
(P, P') = \left(
\begin{bmatrix}
0.6683 & 0.3923 & 0.9669 \\
0.8343 & 0.6885 & 0.8940 \\
0.2613 & 0.2249 & 0.9972
\end{bmatrix}
\begin{matrix} \\ \\, \end{matrix}
\begin{bmatrix}
0.3317 & 0.6077 & 0.0331 \\
0.1657 & 0.3115 & 0.1060 \\
0.7387 & 0.7751 & 0.0028
\end{bmatrix}
\right)
\]

Gaussian Mixtures can be used to gain more fine-grained control over the subnetwork distributions. Assume that a binary matrix $X \in \{0, 1\}^{m \times n}$ is randomly generated and used to index into a probability matrix $P \in \mathbb{R}^{m \times n}$. Using this index matrix $X$, we can sample from Gaussian distributions with different means and variances.

\[
P = \begin{cases}
P_{ij} \sim \mathcal{N}(\mu_1, \sigma_1^2), \ \text{if} \ X_{ij} = 0\\
P_{ij} \sim \mathcal{N}(\mu_2, \sigma_2^2), \ \text{if} \ X_{ij} = 1
\end{cases}
\]

\begin{center}
\begin{tikzpicture}
\begin{axis}[
  no markers, domain=0:1, samples=100,
  axis lines*=left, xlabel=$x$, ylabel=$y$,
  every axis y label/.style={at=(current axis.above origin),anchor=south},
  every axis x label/.style={at=(current axis.right of origin),anchor=west},
  height=5cm, width=12cm,
  xtick={0,1}, ytick=\empty,
  enlargelimits=false, clip=true, axis on top,
  grid = major
  ]
  \addplot [fill=black!20, draw=none, domain=0:1] {gauss(0.25,0.15)} \closedcycle;
  \addplot [very thick,black!50!black] {gauss(0.25,0.15)};
  \addplot [very thick,black!50!black] {gauss(0.75,0.15)};
\end{axis}
\end{tikzpicture}
\end{center}

% Ensembles of these Gaussian subnetworks connect naturally to Deep Gaussian Mixture Models and offer an interesting probabilistic interpretation of neural partitioning. The most generic coefficient of overlap between components follows directly from the mixture definition.

% \[
% MLE_{err} = 1 - \int_0^1 max(\pi_1 f_1(\mu_1, \Sigma_1), ..., \pi_n f_n(\mu_n, \Sigma_n))(x)dx
% \]

\subsubsection{Temperature Scaling}

Temperature scaling may be applied to binary matrices in order to allow for more fine grained control over the stochasticity. Assume that some binary matrix $X \in \{0, 1\}^{m \times n}$ is generated at random. A temperature scaling constant $\tau$ is introduced such that the values in $X$ with a 1 are decayed by $\tau$ and the values with 0 are increased by $\tau$. The mask is then determined on every forward pass with an altered probability according to $\tau$.
%
\begin{gather}
P = \begin{bmatrix}
1-\tau & 1-\tau & 0+\tau & 1-\tau \\
0+\tau & 1-\tau & 0+\tau & 0+\tau \\
1-\tau & 0+\tau & 0+\tau & 1-\tau \\
0+\tau & 0+\tau & 1-\tau & 1-\tau
\end{bmatrix} \\
M = Bernoulli(P)
\end{gather}

Edge-popup is an effective variation on temperature scaling where only the masked values with a 0 are altered by $\tau$. The pre-determined subnetwork is always active, while all the other connections have a small probability to become active on any given forward pass. This offers a regularization effect analagous to dropout in reverse, where the extra dimensionality introduced can allow for optimization benefits and more robust subnetworks.

\begin{gather}
P = \begin{bmatrix}
1 & 1 & 0+\tau & 1 \\
0+\tau & 1 & 0+\tau & 0+\tau \\
1 & 0+\tau & 0+\tau & 1 \\
0+\tau & 0+\tau & 1 & 1
\end{bmatrix} \\
M = Bernoulli(P)
\end{gather}

\subsubsection{Mask Diffusion}

We can further extend temperature scaling with a dynamic annealing schedule. At the beginning of the training process, a high level of stochasticity is desirable as it encourages exploration of the weight space which may help to prevent overfitting and search for more effective subnetwork configurations. As training progresses, the stochasticity should gradually decrease to allow for stable convergence. The annealing function is arbitrary, with some popular examples being the linear, cosine, and exponential decay \cite{}.


\begin{align}
y_{lin}(t) &= \tau_{max} - (\tau_{max} - \tau_{min})  \left( \frac{t}{T_{max}} \right) \\
y_{cos}(t) &= \tau_{min} + \frac{1}{2}(\tau_{max} - \tau_{min}) \left( 1 + cos \left( \frac{t}{T_{max}}\right) \right) \\
y_{exp}(t) &= \tau_{min} + (\tau_{max} - \tau_{min}) e^{- \frac{t}{T_{max}} k}
\end{align}

One formulation of this dynamic temperature scaling results in a process we call mask diffusion, where subnetworks are slowly "revealed" throughout fine-tuning.

All parameters begin with probability 1. Then some subset of probability scores are slowly annealed over the fine tuning phase towards the final subnetwork structure.

Alternatively, the initial probability matrix can be randomized to inject more stochasticity. While this can be leveraged to create highly robust subnetworks, you'd typically need many more training epochs to account for the variability.


\begin{algorithm}
\SetAlgoLined
% \KwIn{N, the number of ensemble members}
\KwIn{($X_{train}, X_{test}$), the training and test data}
\KwIn{($t_{parent}, t_{child}, t_{anneal}$), the number of epochs to train for}
\KwIn{$\phi(\rho)$, the sampling process with target sparsity probability $\rho$}
\KwIn{$\Theta(M, \tau, epoch)$, the temperature scaling function applied to a binary mask $M$ with temperature constant $\tau$}

\texttt{\\}
$F = initialize()$ \\
$F.w = train(F, X_{train}, t_{parent})$ \\
\texttt{\\}
\For{$i$ in $F.layers$}{
    $M_i \sim \phi(\rho)^{F_{i}.w}$ \\
    % $f_{i,j}.w \leftarrow f_{i,j}.w \circ M$ \\
}
\texttt{\\}

\For{$epoch$ in $t_{child}$}{
    \If{$epoch < t_{anneal}$}{
        \For{$i$ in $F.layers$}{
            $P_i \leftarrow \Theta(M_i, \tau, epoch)$ \\
        }
    }
    \texttt{\\}
    \For{$(x, y)$ in $X_{train}$}{
        $F.w \leftarrow F.w \circ Bernoulli(P)$ \\
        $train(F, (x,y))$ \\
    }
}
\texttt{\\}
$F.w \leftarrow F.w \circ M$ \\
$(loss, acc) \leftarrow test(F, X_{test})$ \\
\texttt{\\}
\For{$(x, y)$ in $X_{test}$}{
    $outputs = [f_i(x)\ for\ f_i\ in\ ensemble]$ \\
    $prediction = argmax(mean(outputs))$ \\
}
\caption{Stochastic Mask Annealing}
\end{algorithm}


\section{Experiments}

\subsection{Ablations}

\subsection{Benchmarks}


